The Time-Interlaced Self-Consistent Master System of Heterogeneous-Agent Models

It is shown that the structure of general equilibrium incomplete market models is intrinsically self-consistent and time-interlaced, with mean field interactions that are only implicit and also endogenous. Novel mathematical tools that can handle such structures and do not rely on the representative agent point of view are developed. The study was prompted by the surprising discovery that the common strategy for resolving the classical Aiyagari-Bewley-Huggett model fails to achieve its objective in a widely cited benchmark study. In addition to providing a numerically verifiable solution to such models, the scope of the approximate aggregation conjecture of Krusell and Smith (still an open problem in macroeconomics) is clarified. New features of Krusell-Smith's model are uncovered and novel computational technique, which does not involve simulation, is developed.

==> mac-2.tex <==
%% Time-stamp: <2023-05-12 10:20:21 sglass>
\catcode`@=11
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% Macros for bibliography 
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newtoks\bibm@rk
\newdimen\bibindent%
\newdimen\bibnoskip%

%% the following parameters can be changed before bibliography is printed
\newskip\bibskip%
\bibnoskip=5pt%
\bibskip=0pt%
\bibindent=32pt%
\bibskip=4pt plus 1pt minus 1pt
\def\aut#1{{\rm #1.}}
\def\btitle#1{{\it  #1\/}.}
\def\jtitle#1{{\rm #1.}}
\def\anno#1{({\rm #1}).}
\def\book#1{{\rm #1}}
\def\journal#1 #2 #3{{\it #1\/}~{\bf #2} #3}
\def\journalnt#1 #2 #3{{\it #1\/} {\bf #2} {#3}}
\def\autt#1{{\rm{#1}}}
\def\jjtitle#1{{\rm #1}}




\newcount\@bnumb \newcount\@btot
\@bnumb=0
\@btot=0

\newwrite\@btag
\gdef\ReadWriteBib#1{\openin\@btag \jobname.btag \ifeof\@btag
\relax\else\closein\@btag\relax\input\jobname.btag\fi
\openout\@btag=\jobname.btag\relax\ignorespaces
\global\bibnoskip=#1pt\relax\ignorespaces
\ifnum\the\@btot>0{\setbox0=\hbox{{\the\@btot}.}\global\bibindent=\wd0}\ignorespaces
\global\advance\bibindent by \bibnoskip\else\relax\fi}

\gdef\citeshape#1#2{[\hyperlink{#1}{#2}]}
\gdef\citeshaped#1#2{\hyperlink{#1}{{#2}}}


\gdef\bclust#1#2{\@ifundefined{#1@*@}{\relax}{\ignorespaces
\message{Check cit. [#1]! }\relax}\ignorespaces
\expandafter\gdef\csname \noexpand#1@*@\endcsname{#2}\ignorespaces}

\gdef\cite#1{\@ifundefined{#1@*@}{[#1]\ignorespaces\message{Don't know cit. [#1]!}\ignorespaces
\expandafter\gdef\csname#1@*@\endcsname{#1}\relax}{\citeshape{#1}{\csname#1@*@\endcsname}\relax}\ignorespaces\relax}


\gdef\cited#1{\@ifundefined{#1@*@}{{#1}\ignorespaces\message{Don't know cit. [#1]!}\ignorespaces
\expandafter\gdef\csname#1@*@\endcsname{#1}\relax}{\citeshaped{#1}{\csname#1@*@\endcsname}\relax}\ignorespaces\relax}


\gdef\citel#1{\@ifundefined{#1@*@}{[#1]\ignorespaces\message{Don't know cit. [#1]!}\ignorespaces
\expandafter\gdef\csname#1@*@\endcsname{#1}\relax}{\citeshape{#1}{\csname#1@*@\endcsname}\relax}\ignorespaces\relax}


\gdef\nocite#1#2{\@ifundefined{#1@*@}{[#1]\ignorespaces\message{Don't know cit. [#1]!}\ignorespaces
\expandafter\gdef\csname#1@*@\endcsname{#1}\relax}{\citeshaped{#1}{#2}\relax}\ignorespaces\relax}


\gdef\nonocite#1{\@ifundefined{#1@*@}{\ignorespaces\expandafter\gdef\csname#1@*@\endcsname{#1}\relax}{\relax}\ignorespaces\relax}


\gdef\include#1{\@ifundefined{#1@*@}{\ignorespaces\expandafter\gdef\csname#1@*@\endcsname{#1}\relax}{\relax}\ignorespaces\relax}


%% classic appearance
\iffalse
\gdef\bibshape#1#2{\vskip\bibskip\par\hangindent\bibindent\hangafter1\noindent\ignorespaces
\hbox to\bibindent{\hfill}\ignorespaces
\llap{\relax\hypertarget{#1}{[\bibmark]}\hbox to \bibnoskip{\hfill}}\ignorespaces#2\ignorespaces}

\gdef\bibshapenh#1#2{\vskip\bibskip\par\hangindent\bibindent\hangafter1\noindent\ignorespaces
\hbox to\bibindent{\hfill}\ignorespaces
\llap{[#1]\hbox to \bibnoskip{\hfill}}\ignorespaces#2\ignorespaces}
\fi
%%%%%%%%%%%%%%


\gdef\bibshape#1#2{\vskip\bibskip\par\hangindent\bibindent\hangafter1\noindent\ignorespaces
\hbox to\bibindent{\hfill}\ignorespaces
\llap{\relax\hypertarget{#1}{\bibmark.}\hbox to \bibnoskip{\hfill}}\ignorespaces#2\ignorespaces}

\gdef\bibshapenh#1#2{\vskip\bibskip\par\hangindent\bibindent\hangafter1\noindent\ignorespaces
\hbox to\bibindent{\hfill}\ignorespaces
\llap{{#1.}\hbox to \bibnoskip{\hfill}}\ignorespaces#2\ignorespaces}


\gdef\bibmemo#1{\ignorespaces
\edef\next{\write\@btag{\string\bclust{#1}{\the\bibm@rk}}}\next\ignorespaces}

\gdef\WriteRefTot{\ignorespaces
\edef\next{\write\@btag{\string\SetTotalRefs{\the\@bnumb}}}\next\relax\ignorespaces}

\gdef\SetTotalRefs#1{\global\@btot=#1}

\def\brefitem[#1 (#2)]#3#4\par{\@ifundefined{#3@*@}{\relax}{\global\advance\@bnumb by 1\edef\next{\bibm@rk={\the\@bnumb}}\next\relax\bibmemo{#3}\relax\gdef\bibmark{\csname#3@*@\endcsname}\ignorespaces\bibshape{#3}{#4}}\ignorespaces}

\def\@all@bib[#1 (#2)]#3#4\par{\global\advance\@bnumb by 1\edef\next{\bibm@rk={\the\@bnumb}}\next\relax\@ifundefined{#3@*@}{\bibshapenh{\the\bibm@rk}{#4}}{\bibmemo{#3}\relax\gdef\bibmark{\csname#3@*@\endcsname}\ignorespaces\bibshape{#3}{#4}}\ignorespaces}


\gdef\includeallbref{\let\brefitem\@all@bib\relax}

\catcode`@=12


==> mac-3.tex <==
%% Time-stamp: <2021-12-08 11:34:14 sglass>

\catcode`@=11   %let it be a letter,  so that trics  from plain be used
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcount\@hour
\newcount\@hourmin
\newcount\@minutes

\def\today{\ifcase\month\or
 January\or February\or March\or April\or May\or June\or
 July\or August\or September\or October\or November\or December\fi
 \space\number\day, \number\year}

\newcount\@ye@r


\def\season{\@ye@r=\year\ifnum\@ye@r<2000\advance\@ye@r by -1900\else
\advance\@ye@r by -2000\fi
\ifcase\month\or Spring\or Spring\or Spring\or Spring\or Spring\or Summer\or
 Summer\or Summer\or Fall\or Fall\or Fall\or Fall\fi
 \space'{\ifnum\@ye@r<10\relax0\number\@ye@r\else\relax\number\@ye@r\fi}}
 
\def\calendar{\@ye@r=\year
\ifnum\@ye@r<2000\advance\@ye@r by -1900\else
\advance\@ye@r by -2000\fi\relax\number\month-\ignorespaces
{\ifnum\day<10\relax0\number\day\else\relax\number\day\fi}-\ignorespaces
{\ifnum\@ye@r<10\relax0\number\@ye@r\else\relax\number\@ye@r\fi}\relax}


\def\clock{
\@hour=\time
\divide\@hour by 60
\@hourmin=\@hour
\multiply\@hourmin by 60
\@minutes=\time
\advance\@minutes by -\@hourmin
\ifnum\@hour=0
      \ifnum\@minutes<10
                 12:0\the\@minutes~AM
                       \else 12:\the\@minutes~AM  \fi 
\else  
   \ifnum\@hour<12
           \ifnum\@minutes<10
                 \the\@hour:0\the\@minutes~AM
                       \else \the\@hour:\the\@minutes~AM  \fi
   \else  \ifnum\@hour=12
              \ifnum\@minutes<10
                    \the\@hour:0\the\@minutes~PM
                       \else \the\@hour:\the\@minutes~PM  \fi
           \else \advance\@hour by -12
		    \ifnum\@minutes<10
                    \the\@hour:0\the\@minutes~PM
                       \else \the\@hour:\the\@minutes~PM  \fi \fi \fi \fi \relax}



\def\uclock{
\@hour=\time
\divide\@hour by 60
\@hourmin=\@hour
\multiply\@hourmin by 60
\@minutes=\time
\advance\@minutes by -\@hourmin
\ifnum\@minutes<10
           \the\@hour:0\the\@minutes
                       \else \the\@hour:\the\@minutes\fi
\relax}

\catcode`@=12   %no more a letter 

